Collaborative, Code-Proximal Dynamic Software Visualization within Code Editors

Software visualizations are usually realized as standalone and isolated tools that use embedded code viewers within the visualization. In the context of program comprehension, only few approaches integrate visualizations into code editors, such as integrated development environments. This is surprising since professional developers consider reading source code as one of the most important ways to understand software, therefore spend a lot of time with code editors. In this paper, we introduce the design and proof-of-concept implementation for a software visualization approach that can be embedded into code editors. Our contribution differs from related work in that we use dynamic analysis of a software system's runtime behavior. Additionally, we incorporate distributed tracing. This enables developers to understand how, for example, the currently handled source code behaves as a fully deployed, distributed software system. Our visualization approach enhances common remote pair programming tools and is collaboratively usable by employing shared code cities. As a result, user interactions are synchronized between code editor and visualization, as well as broadcasted to collaborators. To the best of our knowledge, this is the first approach that combines code editors with collaboratively usable code cities. Therefore, we conducted a user study to collect first-time feedback regarding the perceived usefulness and perceived usability of our approach. We additionally collected logging information to provide more data regarding time spent in code cities that are embedded in code editors. Seven teams with two students each participated in that study. The results show that the majority of participants find our approach useful and would employ it for their own use. We provide each participant's video recording, raw results, and all steps to reproduce our experiment as supplementary package.

==> chapters/discussion.tex <==
\section{Discussion}\label{sec:discussion}
In the following, we use the previously presented results to revisit our posed research questions.
Furthermore, we discuss the threats to validity of our evaluation.

\subsection*{\textbf{RQ1}: How long do subjects use the SV and code editor during task solving, respectively?}
TODO

\subsection*{\textbf{RQ2}: Is the code editor perceived as more useful than the SV?}
TODO

\subsection*{\textbf{RQ3}: Are the collaborative SV features perceived as useful?}
TODO

\subsection*{\textbf{RQ4}: Is the approach perceived as useful in the envisioned usage scenarios?}
TODO

\subsection*{\textbf{RQ5}: Is the approach generally perceived as usable?}
TODO

\subsection{Threats to Validity}

\begin{itemize}
	\item Small Visualization: (Have to take experience level into account,  experiment is addressed to undergraduates with less experience in web development)
	\item Little communication in experiment (real life: filtering~\cite{bassil2001,kienle2007} would achieve something similar)
	\item small sample size (our study’s sample size is higher than the median participant count (13) and ranks among the most usual sample sizes in the related SV literature body~\cite{merino2018}
	\item Low Distribution (See 22 + X groups were randomly assigned)
\end{itemize}

